Factor system for graphs and combinatorial HHS

We relaxe the constraint on the domains of combinatorial HHS machinery so combinatorial HHS machinery works for most cubical curve graphs. As an application we extend the factor system machinery of the CAT(0) cube complex to the quasi-median graphs.

==> bibilography.tex <==
@article{BHMS20,
	title={A combinatorial take on hierarchical hyperbolicity and applications to quotients of mapping class groups},
	author={Behrstock, Jason and Hagen, Mark and Martin, Alexandre and Sisto, Alessandro},
	journal={arXiv preprint arXiv:2005.00567},
	year={2020}
}

@article{BR20,
	title={Hierarchical hyperbolicity of graph products},
	author={Berlyne, Daniel and Russell, Jacob},
	journal={arXiv preprint arXiv:2006.03085},
	year={2020}
}

@article{HS20,
	title={On hierarchical hyperbolicity of cubical groups},
	author={Hagen, Mark F and Susse, Tim},
	journal={Israel Journal of Mathematics},
	pages={1--45},
	year={2020},
	publisher={Springer}
}

@article{Gen17,
	title={Cubical-like geometry of quasi-median graphs and applications to geometric group theory},
	author={Genevois, Anthony},
	journal={arXiv preprint arXiv:1712.01618},
	year={2017}
}

@article{BHS17,
	title={Hierarchically hyperbolic spaces, I: Curve complexes for cubical groups},
	author={Behrstock, Jason and Hagen, Mark and Sisto, Alessandro},
	journal={Geometry \& Topology},
	volume={21},
	number={3},
	pages={1731--1804},
	year={2017},
	publisher={Mathematical Sciences Publishers}
}

@article{BHS19,
	title={Hierarchically hyperbolic spaces II: Combination theorems and the distance formula},
	author={Behrstock, Jason and Hagen, Mark and Sisto, Alessandro},
	journal={Pacific Journal of Mathematics},
	volume={299},
	number={2},
	pages={257--338},
	year={2019},
	publisher={Mathematical Sciences Publishers}
}

@article{Vok17,
	title={Hierarchical hyperbolicity of graphs of multicurves},
	author={Vokes, Kate M},
	journal={arXiv preprint arXiv:1711.03080},
	year={2017}
}

@article{HMS21,
	title={Extra-large type Artin groups are hierarchically hyperbolic},
	author={Hagen, Mark and Martin, Alexandre and Sisto, Alessandro},
	journal={arXiv preprint arXiv:2109.04387},
	year={2021}
}

@article{Val18,
	title={Acylindrical hyperbolicity of groups acting on quasi-median graphs and equations in graph products},
	author={Valiunas, Motiejus},
	journal={arXiv preprint arXiv:1811.02975},
	year={2018}
}

@article{ber21,
	title={Hierarchical Hyperbolicity of Graph Products and Graph Braid Groups},
	author={Berlyne, Daniel James Solomon},
	year={2021}
}

@article{Sa95,
	title={Ends of group pairs and non-positively curved cube complexes},
	author={Sageev, Michah},
	journal={Proceedings of the London Mathematical Society},
	volume={3},
	number={3},
	pages={585--617},
	year={1995},
	publisher={Oxford Academic}
}

@article{CN05,
	title={From wall spaces to CAT (0) cube complexes},
	author={Chatterji, Indira and Niblo, Graham},
	journal={International Journal of Algebra and Computation},
	volume={15},
	number={05n06},
	pages={875--885},
	year={2005},
	publisher={World Scientific}
}

@article{BR18,
	title={A refined combination theorem for hierarchically hyperbolic groups},
	author={Berlai, Federico and Robbio, Bruno},
	journal={Groups, Geometry, and Dynamics},
	volume={14},
	number={4},
	pages={1127--1203},
	year={2020}
}

@article{ABM21,
	title={Largest acylindrical actions and stability in hierarchically hyperbolic groups},
	author={Abbott, Carolyn and Behrstock, Jason and Durham, Matthew},
	journal={Transactions of the American Mathematical Society, Series B},
	volume={8},
	number={3},
	pages={66--104},
	year={2021}
}

@article{CS11,
	title={Rank rigidity for CAT (0) cube complexes},
	author={Caprace, Pierre-Emmanuel and Sageev, Michah},
	journal={Geometric and functional analysis},
	volume={21},
	number={4},
	pages={851--891},
	year={2011},
	publisher={Springer}
}

@article{GM19,
	title={Automorphisms of graph products of groups from a geometric perspective},
	author={Genevois, Anthony and Martin, Alexandre},
	journal={Proceedings of the London Mathematical Society},
	volume={119},
	number={6},
	pages={1745--1779},
	year={2019},
	publisher={Wiley Online Library}
}

@article{Man05,
	title={Geometry of pseudocharacters},
	author={Manning, Jason Fox},
	journal={Geometry \& Topology},
	volume={9},
	number={2},
	pages={1147--1185},
	year={2005},
	publisher={Mathematical Sciences Publishers}
}

@article{HMS23,
	title={A Combinatorial Structure for Many Hierarchically Hyperbolic Spaces},
	author={Hagen, Mark and Mangioni, Giorgio and Sisto, Alessandro},
	journal={arXiv preprint arXiv:2308.16335},
	year={2023}
}

@article{DDLS21,
	title={Extensions of Veech groups II: hierarchical hyperbolicity and quasi-isometric rigidity},
	author={Dowdall, Spencer and Durham, Matthew G and Leininger, Christopher J and Sisto, Alessandro},
	journal={arXiv preprint arXiv:2111.00685},
	year={2021}
}

@article{Rus21,
	title={Extensions of multicurve stabilizers are hierarchically hyperbolic},
	author={Russell, Jacob},
	journal={arXiv preprint arXiv:2107.14116},
	year={2021}
}

